Characterising the true descendants of the first stars

The metal-poor stars in the Galactic halo are thought to show the imprints of the first (PopIII) stars, and thus provide a glance at the first episodes of star formation. In this work, we aim at understanding whether all very metal-poor stars formed in environments polluted by PopIII supernovae (SNe) and at what level. With a general parametric model for early metal enrichment, we study the chemical abundances (from C to Zn) of an environment imprinted by a single PopIII SN. We investigate how these abundances depend on the initial mass and internal mixing of PopIII stars, as well as on their SN explosion energy. We then study how subsequent generations of normal (PopII) SNe affect the PopIII chemical signatures. By comparing the observed chemical abundances with our model predictions, we show that stars with [C/Fe]$>+2.5$ form in environments polluted purely by low-energy PopIII SNe ($E_{\rm SN}<2\times 10^{51}$erg). At lower [C/Fe], stars can be imprinted either by PopIII only, or also by normal PopII SNe. The probability of being enriched by PopII SNe increases as [C/Fe] decreases. When PopII stars contribute more to the pollution, they wash out the diverse chemical peculiarities left by the different PopIII SNe, and the chemical dispersion between their descendants decreases. We conclude that C-normal stars ($\rm [C/Fe] \leq +0.7$) have likely been enriched by PopII SNe at a $\geq 50\%$ level and we identify in the abundance scatter a key diagnostic to pinpoint the signature of PopIII SNe.

==> Model/model.tex <==
\section{Methods}

The parametric model described in \citet{Salvadori2019} follows the chemical evolution of a primordial mini-halo after the birth and explosion of the first two stellar generations, the first of which is composed only by primordial Pair Instability Supernovae\footnote{A Pair Instability Supernova is the final life stage of a star with initial mass between $140 M_{\odot}$ and $260M_{\odot}$. This kind of SN has an energy between $10^{52}$ and $10^{53} erg$.} (PISN). However, this kind of model is general and it can be applied to different cases, as we will explain in this Section.


In this Section we resume the original chemical evolution model as described in \citet{Salvadori2019} and then we work out its implementation. 

\subsection{The original model}
\label{sec:original}

We will summarize here the principal features of the parametric model in \citet{Salvadori2019}.

Mini-halos are defined as dark matter halos with a virial temperature, $T_{vir}$, lower than $2 \times 10^4 K$. Primordial mini-halos are composed only of hydrogen and helium and, given their low temperatures, the only way they can cool down gas to form stars is with molecular hydrogen, $H_2$. The cooling efficiency of this mechanism depends on $T_{vir}$, the gas density and the virialization redshift, $z$, and it affects the star formation efficiency (SFE), $f_*$, of the mini-halo. $f_*$, in turn, depends on $T_{vir}$ and it can be expressed as (see \citet{Salvadori2009a}):

\begin{equation}
	\label{fstar}
	f_*(T_{vir})=\dfrac{2\times f_*^{Ly\alpha-cool}}{[1+(2\times10^4K/T_{vir})^3]},
\end{equation} 

where $f_*^{Ly\alpha-cool}$ is the SFE of a Lyman $\alpha$ cooling primordial halo with a virial temperature of $2 \times 10^4 K$ and it is supposed to be $0.1$. The minimum virial temperature for a primordial mini-halo to cool down its gas and form stars is $2 \times 10^3 K$ (e.g. \citet{Tegmark1997}), thus, for primordial mini-halos, $f_* \in [10^{-4}; 10^{-1}]$. 

The virial mass of a mini-halo is linked with its virial temperature and the virialization redshift by this equation from \citet{Barkana2001}:

\begin{equation}
	\label{Tvir}
	T_{vir}=1.98\times10^4 K\, \left(\frac{\mu}{0.6}\right)\,\left(\frac{1+z}{10}\right)\,\left(\frac{M}{10^8\,h^{-1}\,M_{\odot}}\right)^{2/3};
\end{equation}

$\mu$ is the mean molecular weight of the gas, $\mu=1.22$ for molecular and $\mu=0.59$ for atomic gas. Using this equation with $z=10$, we end up with primordial mini-halos with virial masses between $10^{6.5}$ and $10^8 M_{\odot}$. The mass of the gas inside a mini-halo with virial mass $M_h$ is calculated as $M_g=\dfrac{\Omega_b}{\Omega_m}M_h$. Assuming that the stars of the first generation form all together in an unique burst, the total stellar mass formed is calculated as $M_{burst}=f_*\,M_g$. The metals synthesized and ejected in the ISM by the first generation of stars can be diluted in a small fraction of the primordial gas content of the mini-halo or even ejected out of its virial radius, depending on the explosion energy of the stars, the virial mass and the density of the mini-halo. This uncertainty is enclosed in a parameter, $f_{dil}=f_g/f_Z$, where $f_g$ is the mini-halo gas fraction where metals are diluted and $f_Z$ is the fraction of metals retained in the galaxy. $f_{dil}$ has values between $0.08$ and $10$: if $f_{dil} < 1$, all the ejected metals are retained in the galaxy and they are diluted in a fraction of the total gas, if $f_{dil} > 1$, there are two possible events: a part of the ejected metals is pushed out of the halo and/or pristine gas gets accreted.

The abundance of a chemical element X with respect to hydrogen in the ISM of the hosting mini-halo, after the first generation of stars exploded, is

\begin{equation}
	\label{XsuHiii}
	\left[\dfrac{X}{H}\right]_{ISM}=\log\left[\dfrac{f_*}{f_{dil}}\,Y_X^{PopIII}\right]-\log\left[\dfrac{M_{X, \odot}}{M_{H, \odot}}\right],
\end{equation}

where $Y_X^{PopIII}$ is the yield of the chemical element X and $M_{X, \odot}$ ($M_{H, \odot}$) is the mass of the element X (hydrogen) in the photosphere of the Sun.

The abundance of an element X with respect to iron is

\begin{equation}
	\label{XsuFeiii}
	\left[\dfrac{X}{Fe}\right]_{ISM}=\log\left[\dfrac{Y_X^{PopIII}}{Y_{Fe}^{PopIII}}\right]-\log\left[\dfrac{M_{X, \odot}}{M_{Fe, \odot}}\right].
\end{equation}

Since PopIII star formation models predict that they were likely very massive, up to $1000 M_{\odot}$ (e.g. \citet{Bromm2001}), they must have ended their lives in few million years. After the explosion of the first generation of stars, the ISM metallicity usually overcomes the critical metallicity, $Z_{cr}\sim 10^{-4.5} Z_{\odot}$, (see \citet{DeBennassuti2017}) and normal PopII stars can form. 

PopII stars, which explode at different times depending on their initial mass (see \citet{Raiteri1996a}), enrich the ISM with the chemical elements they synthesized: the fraction of metals ejected by PopIII stars with respect to the total amount of metal in the ISM is expressed by $f_{PopIII}$ and the yield of a chemical element X, $Y_X^{PopII}(t, Z_{ISM})$, grows as time passes.

The SFE of PopII stars can be computed retrospectively as $f_*^{PopII}=\dfrac{f_*}{f_{dil}}\dfrac{Y_Z^{PopIII}}{Y_Z^{PopII}}\dfrac{1-f_{PopIII}}{f_{PopIII}}$ (see \citet{Salvadori2019} for further details), and it must be less than $0.1$ (see \citet{Pallottini2017}).

At every time step after the formation of PopII stars we can compute the ISM chemical abundances with this two equations:

\begin{equation}
	\label{XsuH_II}
	[X/H]_{ISM}=\log\left[\frac{f_*}{f_{dil}} Y_X^{PopIII}+f_*^{PopII}\,Y_X^{PopII}\right]-\log\left[\frac{M_{X, \odot}}{M_{H, \odot}}\right],
\end{equation}

\begin{equation}
	\label{XsuFe_II}
	[X/Fe]_{ISM}=\log\left[\dfrac{\frac{f_*}{f_{dil}} Y_X^{PopIII}+f_*^{PopII}\,Y_X^{PopII}}{\frac{f_*}{f_{dil}} Y_{Fe}^{PopIII}+f_*^{PopII}\,Y_{Fe}^{PopII}}\right]-\log\left[\frac{M_{X, \odot}}{M_{Fe, \odot}}\right].
\end{equation}



\subsection{Model implementation}

In order to explain the origins of metal-poor halo stars, we must investigate the chemical enrichment of the first star forming mini-halos, which are the best candidates for hosting the oldest and most metal-poor stars. Thus, in this Section, we will explain the improvements we made to the original model to reach our goal.

\subsubsection{Cosmological context}

We define the cosmological context\footnote{We use a $\Lambda-CDM$ model with cosmological parameters from \citet{Aghanim2020}: $h=0.669, \Omega_m=0.31, \Omega_bh^2=0.02, \Omega_{\Lambda}=0.69, \sigma_8=0.8, n=0.97$.} by assuming that halos comoving densities follow the Extended Press\&Schecter theory (EPS theory, see \citet{Press1974}, \citet{Bond1991}). We suppose that the star formation in our mini-halos happens at $z\sim10$ and that the total comoving volume is the same as the Milky Way comoving volume, $V=1 Mpc^3$. We compute the number of mini-halos for $20$ virial temperatures (and corresponding virial masses) between $2\times10^3 K$ and $2\times10^4 K$ multiplying their comoving density by $V$.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Model/Images/Press_log.png}
    \caption{Number of mini-halos (red line) and star formation rate (blue rate) as a function of virial temperature, $T_{vir}$, or virial mass, $M_{vir}$, of the halo at redshift $z=10$.}
    \label{fig:press_log}
\end{figure}

We show in figure \ref{fig:press_log} with the red line the derived number of mini-halos, $N_{halo}$, with respect to their virial temperature or mass. The total number of mini-halos is $\sim 1600$. 

\subsubsection{IMF exploration and sampling}

The IMF of the first stars is still a debated question. Given the high central temperature of primordial collapsing clouds we would expect that PopIII stars were very massive. Indeed some simulations (e.g. \citet{Bromm2002}, \citet{Hirano2014}) find that, in absence of turbulence and magnetic fields, primordial stars could have masses up to $1000 M_{\odot}$. Yet, if we also consider the presence of a magnetic field in 3D simulations, the resulting mass range is moved to smaller masses, till $0.1 M_{\odot}$ (see \citet{Greif2011}). However, this kind of simulations can follow the accretion process just for a small fraction of the star formation time scale, thus the small fragments can later merge together to form a heavier star (e.g. \citet{Hirano2017}). 

To cover this wide range of possibilities, PopIII stars are believed to have masses between $0.1 M_{\odot}$ and $1000 M_{\odot}$. However, if PopIII stars with masses lower than $0.8 M_{\odot}$ had formed, they should be still alive and observable nowadays in the oldest and most metal-poor systems of the Local Group (see \citet{Rossi2021}). The fact that we never observed a zero-metallicity star in the stellar halo of the Milky Way nor in an ultra-faint dwarf galaxy has two possible explanations: PopIII stars are really rare and we haven't yet observed enough stars to find one of them, or their masses were greater than $0.8 M_{\odot}$. 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Model/Images/Sampling_IMF.pdf}
    \caption{Sampled (coloured bars) versus theoretical (black dashed line) normalized IMF for three different cases. From \emph{left} to \emph{right} panel: Larson's type IMF with $m_{ch}=1 M_{\odot}$, same with $m_{ch}=100 M_{\odot}$ and flat IMF. All of them are computed to get a total stellar burst of $M_{burst}= 1000 M_{\odot}$, with stellar masses in the range $[0.8 M_{\odot}; 1000 M_{\odot}]$.}
    \label{fig:Sampling_IMF}
\end{figure*}

We then assume that PopIII stellar masses have values in the range $[0.8 M_{\odot}; 1000 M_{\odot}]$ and two different IMF shapes: a normalized Larson's type\footnote{$\Phi(m)\propto \left(\frac{m}{m_{ch}}\right)^{\alpha-1}e^{-m_{ch}/m}$} with $\alpha=-1.35$ and $m_{ch}=1 M_{\odot}$ or $m_{ch}= 100 M_{\odot}$ and a flat IMF (they are shown in figure \ref{fig:Sampling_IMF} with the dashed lines). 

When dealing with small halos, we must take into account a sampled IMF (e.g. \citet{DeBennassuti2017}, \citet{Rossi2021}). Indeed, given their low star formation efficiency, the total stellar mass formed in a star-formation burst, $M_{burst}$, might be smaller than the maximum initial mass we assumed for PopIII stars, $1000 M_{\odot}$, and very massive stars will likely not form in primordial mini-halos. Thus, the IMF for PopIII stars is not a continuous function, but it depends on the gas availability and the virial temperature of every mini-halo. The IMF sampling, as performed in \citet{Rossi2021}, is based on a Monte Carlo procedure: a random mass $M_*^i$ is extracted, following the IMF probability, until the total stellar mass formed, $\sum_i N_*^i M_*^i$, is equal to $M_{burst}$, where $N_*^i$ is the number of star with mass $M_*^i$. We evaluate the Star Formation Rate (SFR) as the stellar burst mass dividev by the free fall time, $\Psi=\dfrac{M_{burst}}{t_{ff}}$, where $t_{ff}=\left(\dfrac{3\,\pi}{32\,G\,\rho}\right)^{1/2}\approx 50 Myr$ at $z=10$. The results of this computation are shown in the figure \ref{fig:press_log} with the blue line and are consistent with \citet{Rossi2021}.

We present how the sampling procedure acts on a normalized Larson IMF in figure \ref{fig:Sampling_IMF}. Comparing the sampled IMF of the left and middle panels (bars) with the theoretical Larson IMF (dashed line), we can see that the incomplete IMF sampling is more pronounced for higher $m_{ch}$. This is because for increasing characteristic mass, halos tend to form heavier stars, reaching the total stellar mass formed, $M_{burst}$, with a limited number of stars, which have masses near the IMF peak. This is even more pronounced for a flat IMF because very massive stars have the same probability to form as low mass stars. When applying the EPS theory, the number of halos strongly decreases for increasing halo mass (see figure \ref{fig:press_log}). For this reason, the overall effect on the main mini-halo population is a truncation of the true PopIII IMF at $M_*\approx 100 M_{\odot}$ when $m_{ch}=1M_{\odot}$. 

For every mass bin, the sampling procedure provides us with the total number of stars formed, $N_*^i$. Since the total mass of an element $X$ formed in a halo is $m_X=\sum_i\,Y_X^i\,M_*^i\,N_*^i$, we can compute the total yield per stellar burst as $Y_X=m_X/M_{burst}$, where $m_X=\sum_i\,Y_X^i\,M_*^i\,N_*^i$, $M_{burst}=\sum_i N_*^i M_*^i$ and $Y_X^i$ is the yield of the element $X$ per stellar mass $M_*^i$. \\



MANCA PARTE POPII



\subsubsection{Mechanical feedback}

For everyone of our twenty virial temperatures, or halo masses, we computed the binding energy using the equation \ref{ebind}. When one or some supernovae explode in a halo, their explosion energy is turned in thermal and kinetic energy of the surrounding gas. Gas can eventually be heated up and, expanding, it can escape the virial radius of the halo. However, we didn't take into account of this effect. We evaluated the gas kinetic energy as $E_{kin}=f_{kin} \sum_{i=1}^{N_{SN}^i}E_{SN}^i= f_{kin}\,E_{SN}^{tot}$, where $f_{kin}$ has an unknown value between $0.01$ and $0.1$ and we consider the cumulative explosion of all SNe, of energy $E_{SN}^{tot}$. It means that, when $f_{kin}=0.01$ we have the minimum kinetic energy of the gas and the maximum thermal energy; we suppose that, in this case, if $E_{kin} > E_{bind}$, the gas is completely ejected out of the virial radius of the halo, which is disrupted and stops forming stars. On the opposite side, if $E_{kin} < E_{bind}$, the halo survives and forms another generation of stars.









==> Model/simple_model.tex <==
\section{Methods}

The parametric model described in \citet{Salvadori2019} follows the chemical evolution of a primordial mini-halo after the birth and explosion of the first two stellar generations, the first of which is composed only by primordial Pair Instability Supernovae\footnote{A Pair Instability Supernova is the final life stage of a star with initial mass between $140 M_{\odot}$ and $260M_{\odot}$. This kind of SN has an energy between $10^{52}$ and $10^{53} erg$.} (PISN). However, this kind of model is general and it can be applied to a broader range of stellar masses, as we will explain in this Section.

In this Section we resume the original chemical evolution model as described in \citet{Salvadori2019}. 

\subsection{The original model}
\label{sec:original}

We will summarize here the principal features of the parametric model in \citet{Salvadori2019}.

Mini-halos are defined as dark matter halos with a virial temperature, $T_{vir}$, lower than $2 \times 10^4 K$. Primordial mini-halos are composed only of hydrogen and helium and, given their low temperatures, the only way they can cool down gas to form stars is with molecular hydrogen, $H_2$. The cooling efficiency of this mechanism depends on $T_{vir}$, the gas density and the virialization redshift, $z$, and it affects the star formation efficiency (SFE), $f_*$, of the mini-halo. $f_*$, in turn, depends on $T_{vir}$ and it can be expressed as (see \citet{Salvadori2009a}):

\begin{equation}
	\label{fstar}
	f_*(T_{vir})=\dfrac{2\times f_*^{Ly\alpha-cool}}{[1+(2\times10^4K/T_{vir})^3]},
\end{equation} 

where $f_*^{Ly\alpha-cool}$ is the SFE of a Lyman $\alpha$ cooling primordial halo with a virial temperature of $2 \times 10^4 K$ and it is supposed to be $0.1$. The minimum virial temperature for a primordial mini-halo to cool down its gas and form stars is $2 \times 10^3 K$ (e.g. \citet{Tegmark1997}), thus, for primordial mini-halos, $f_* \in [10^{-4}; 10^{-1}]$. 

The virial mass of a mini-halo is linked with its virial temperature and the virialization redshift by this equation from \citet{Barkana2001}:

\begin{equation}
	\label{Tvir}
	T_{vir}=1.98\times10^4 K\, \left(\frac{\mu}{0.6}\right)\,\left(\frac{1+z}{10}\right)\,\left(\frac{M}{10^8\,h^{-1}\,M_{\odot}}\right)^{2/3};
\end{equation}

$\mu$ is the mean molecular weight of the gas, $\mu=1.22$ for molecular and $\mu=0.59$ for atomic gas. Using this equation with $z=10$, we end up with primordial mini-halos with virial masses between $10^{6.5}$ and $10^8 M_{\odot}$. The mass of the gas inside a mini-halo with virial mass $M_h$ is calculated as $M_g=\dfrac{\Omega_b}{\Omega_m}M_h$. Assuming that the stars of the first generation form all together in an unique burst, the total stellar mass formed is calculated as $M_{burst}=f_*\,M_g$. The metals synthesized and ejected in the ISM by the first generation of stars can be diluted in a small fraction of the primordial gas content of the mini-halo or even ejected out of its virial radius, depending on the explosion energy of the stars, the virial mass and the density of the mini-halo. This uncertainty is enclosed in a parameter, $f_{dil}=f_g/f_Z$, where $f_g$ is the mini-halo gas fraction where metals are diluted and $f_Z$ is the fraction of metals retained in the galaxy. $f_{dil}$ has values between $0.08$ and $10$: if $f_{dil} < 1$, all the ejected metals are retained in the galaxy and they are diluted in a fraction of the total gas, if $f_{dil} > 1$, there are two possible events: a part of the ejected metals is pushed out of the halo and/or pristine gas gets accreted.

The abundance of a chemical element X with respect to hydrogen in the ISM of the hosting mini-halo, after the first generation of stars exploded, is

\begin{equation}
	\label{XsuHiii}
	\left[\dfrac{X}{H}\right]_{ISM}=\log\left[\dfrac{f_*}{f_{dil}}\,Y_X^{PopIII}\right]-\log\left[\dfrac{M_{X, \odot}}{M_{H, \odot}}\right],
\end{equation}

where $Y_X^{PopIII}$ is the yield of the chemical element X and $M_{X, \odot}$ ($M_{H, \odot}$) is the mass of the element X (hydrogen) in the photosphere of the Sun.

The abundance of an element X with respect to iron is

\begin{equation}
	\label{XsuFeiii}
	\left[\dfrac{X}{Fe}\right]_{ISM}=\log\left[\dfrac{Y_X^{PopIII}}{Y_{Fe}^{PopIII}}\right]-\log\left[\dfrac{M_{X, \odot}}{M_{Fe, \odot}}\right].
\end{equation}

Since PopIII star formation models predict that they were likely very massive, up to $1000 M_{\odot}$ (e.g. \citet{Bromm2001}), they must have ended their lives in few million years. After the explosion of the first generation of stars, the ISM metallicity usually overcomes the critical metallicity, $Z_{cr}\sim 10^{-4.5} Z_{\odot}$, (see \citet{DeBennassuti2017}) and normal PopII stars can form. 

PopII stars, which explode at different times depending on their initial mass (see \citet{Raiteri1996a}), enrich the ISM with the chemical elements they synthesized: the fraction of metals ejected by PopIII stars with respect to the total amount of metal in the ISM is expressed by $f_{PopIII}$ and the yield of a chemical element X, $Y_X^{PopII}(t, Z_{ISM})$, grows as time passes.

The SFE of PopII stars can be computed retrospectively as $f_*^{PopII}=\dfrac{f_*}{f_{dil}}\dfrac{Y_Z^{PopIII}}{Y_Z^{PopII}}\dfrac{1-f_{PopIII}}{f_{PopIII}}$ (see \citet{Salvadori2019} for further details), and it must be less than $0.1$ (see \citet{Pallottini2017}).

At every time step after the formation of PopII stars we can compute the ISM chemical abundances with this two equations:

\begin{equation}
	\label{XsuH_II}
	[X/H]_{ISM}=\log\left[\frac{f_*}{f_{dil}} Y_X^{PopIII}+f_*^{PopII}\,Y_X^{PopII}\right]-\log\left[\frac{M_{X, \odot}}{M_{H, \odot}}\right],
\end{equation}

\begin{equation}
	\label{XsuFe_II}
	[X/Fe]_{ISM}=\log\left[\dfrac{\frac{f_*}{f_{dil}} Y_X^{PopIII}+f_*^{PopII}\,Y_X^{PopII}}{\frac{f_*}{f_{dil}} Y_{Fe}^{PopIII}+f_*^{PopII}\,Y_{Fe}^{PopII}}\right]-\log\left[\frac{M_{X, \odot}}{M_{Fe, \odot}}\right].
\end{equation}











==> Results/results.tex <==
\section{Results}
\label{results}

\subsection{Only PopIII stars, varying their explosion energy}

\begin{figure}
    \centering
    \includegraphics[width=0.65\columnwidth]{Results/Images/Flat_oneEn.pdf}
    \caption{Caption}
    \label{fig:flat_oneen}
\end{figure}

\subsection{Only PopIII stars, varying their IMF}
\subsubsection{Larson's IMF with $m_{ch}=1M_{\odot}$ and $m_{ch}=100M_{\odot}$}
\subsubsection{Flat IMF}

\subsection{After the contribution of PopII stars}

==> Results/results_simple.tex <==
\section{A simple parametric study}

We start with the simplest case. Our mini-halos are enriched by PopIII stars with a delta function IMF\footnote{$\Phi(M_*)=A \times \delta(M_*)$, where $A$ is a normalization constant.} with stellar masses $M_*\in[10; 100] M_{\odot}$ and $M_*\in[140; 260] M_{\odot}$. The stars with initial masses in the first range explode as supernovae (SN) with ten different energies, $E_{SN} \in [0.3 ; 10] \times 10^{51} erg$, which we split in four categories, as done in \citet{Cooke2014}: faint SN when $E_{SN} \in [0.3; 0.6] foe$\footnote{$1 foe=10^{51} erg$}, core-collapse (CC) SN when $E_{SN} \in [0.9; 1.5] foe$, high-energy (HE) SN when $E_{SN} \in [1.8; 3.0] foe$ and hypernovae when $E_{SN} \in [5.0; 10.0] foe$. If we assume a delta function IMF, one star, or more with the same initial masses, explodes in each mini-halo. 

Following the prescriptions of \citet{Salvadori2019}, we have $f_*/f_{dil} \in [10^{-4}; 10^{-1}]$ for mini-halos with virial temperatures $T_{vir} \in [0.2; 2] \times 10^4 K$. 

After the enrichment of the first stellar generation, the metallicity of the ISM overcomes the critical metallicity and normal PopII stars can be formed. We assume that their initial masses are distributed as a Larson IMF\footnote{$\Phi(M_*)=A M_*^{-2.35} \exp\left(-\dfrac{m_{ch}}{M_*}\right)$, where A is a normalization constant and $m_{ch}$ is the characteristic mass.} with $m_{ch}=0.35 M_{\odot}$ and we only account for the stars that explode as core-collapse supernovae with masses $M_* \in [8; 40] M_{\odot}$ and $E_{SN} \sim 10^{51} erg$.\\

{\bf STEF: Here, or perhaps even before, you should add the figure showing the assumed mass range of Pop~III stars and the corresponding explosion energy of SNe}

\subsection{Results}

We will now present the key chemical properties of mini-halos, firstly, enriched only by PopIII SNe with different energies and, secondly, by core-collapse SNe of a second stellar generation. 

\subsubsection{Chemical enrichment of PopIII SNe}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{Results/Images/ISM_1.pdf}
    \caption{ISM abundances, $[X/Fe] vs. [Fe/H]$, after the explosion of the first generation of stars for some key chemical elements (in each column), carbon, oxygen and magnesium, with different explosion energies of the first stars (in each row). The IMF of the first stars is a delta function and the color of each area represents the probability of having these abundances. The diagrams in the first four rows are for mini-halos enriched by stars which explode as \emph{normal} SNe, while the last row is for mini-halos enriched by PISN. In each diagram we also represented the chemical abundances of the observed carbon-enhanced (carbon-normal) metal-poor halo stars with black filled (empty) star-shaped points (see Section observations) and we used arrows to denote the upper or lower limits.}
    \label{fig:popiii_delta_1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Results/Images/ISM_2.pdf}
    \caption{The same as figure \ref{fig:popiii_delta_1}, but for aluminum, silicon and calcium.} 
    \label{fig:popiii_delta_2}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Results/Images/ISM_3.pdf}
    \caption{The same as figures \ref{fig:popiii_delta_1} and \ref{fig:popiii_delta_2}, but for titanium, manganese, zinc.}
    \label{fig:popiii_delta_3}
\end{figure*}

\textcolor{red}{SECONDO ME DOVREI COMMENTARE INSIEME LE FIGURE CON LE MASSE E QUELLE CON I CONTOUR, COSì POSSO SPIEGARE IL FATTO CHE SI HANNO ALTI C/Fe SOLO QUANDO ESPLODONO FAINT MASSICCE.}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Results/Images/ISM_masses1.pdf}
    \caption{ISM abudances, $[X/Fe] vs. [Fe/H]$, after the explosion of the first generation of stars for some key chemical elements (in each column), carbon, oxygen and magnesium, with different explosion energies of the first stars (in each row). We differentiate the abundances for different initial stellar masses, from blue, the lighter ones, to green, the heavier one. The IMF of the first stars is a delta function and the color of each area represents the probability of having these abundances. The diagrams in the first two rows are for mini-halos enriched by stars which explode as \emph{normal} SNe, while the last row is for mini-halos enriched by PISN. In each diagram we also represented the chemical abundances of the observed carbon-enhanced (carbon-normal) metal-poor halo stars with black filled (empty) star-shaped points (see Section observations) and we used arrows to denote the upper or lower limits.}
    \label{fig:popiii_masses_1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Results/Images/ISM_masses2.pdf}
    \caption{The same as figure \ref{fig:popiii_masses_1}, but for aluminum, silicon and calcium.} 
    \label{fig:popiii_masses_2}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Results/Images/ISM_masses3.pdf}
    \caption{The same as figures \ref{fig:popiii_masses_1} and \ref{fig:popiii_masses_2}, but for titanium, manganese, zinc.}
    \label{fig:popiii_masses_3}
\end{figure*}


In figures \ref{fig:popiii_delta_1}, \ref{fig:popiii_delta_2} and \ref{fig:popiii_delta_3} we represent the chemical abundances for some key chemical elements compared to the abundance of iron, $[Fe/H]$, when the mini-halos are enriched only by PopIII SNe, using the results of the equations \ref{XsuHiii} and \ref{XsuFeiii}. The plots in the first four rows are for $M_* \in [10; 100] M_{\odot}$ (\emph{normal} SNe range), while the plots in the last row are for $M_* \in [140; 260] M_{\odot}$ (PISN range). Choosing a delta function IMF and dividing the results for different explosion energies, the ISM abundances of each mini-halo depend only on the initial mass of the stars, and we will come back on this point later, and the value of $f_*/f_{dil}$. Indeed, if we inspect equations \ref{XsuHiii} and \ref{XsuFeiii} we can see that they depend on $Y_{X}^{PopIII}$, which depends only on the masses of the stars that explode in the mini-halo and their explosion energies, and on $f_*/f_{dil}$, for which we chose ten representative values in the already mentioned range. Different values of $f_*/f_{dil}$ affect $[Fe/H]$, but not $[X/Fe]$. We will firstly comment (\textcolor{red}{si dice così?}) on the results we get when $M_* \in [10; 100] M_{\odot}$, focusing on the plots in the first four rows of each figure. 

The overall trend with increasing explosion energy, increasing from the left to the right columns in figure \ref{fig:onlypopiii_delta}, is an increase in $[Fe/H]$ and a decrease in $[X/Fe]$ for most of the chemical elements. This is due to the fact that low-energy SNe experience a strong fall-back and expel only the most external shells of the star. That's also why $[Fe/H]$ reaches very low values, up to $-8$, only when low-energy SNe explode in the mini-halos. However, the upper limit of $[Fe/H]$ is always higher that $-1$.

Focusing on the lighter elements like C, O and Mg, $[X/Fe] > 3$ can be reached only with the explosions of faint SNe and CC SNe.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Results/Images/Carbon_popII.pdf}
    \caption{}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Results/Images/All_popII-1.pdf}
    \caption{}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Results/Images/All_popII-2.pdf}
    \caption{}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Results/Images/CEMP_4_6_new.pdf}
    \caption{CEMP con [Fe/H] tra -6 e -4}
    \label{fig:CEMP_4_6}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Results/Images/CEMP_2_4.pdf}
    \caption{CEMP con [Fe/H] tra -4 e -2}
    \label{fig:CEMP_2_4}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Results/Images/MP_2_4.pdf}
    \caption{C-norm con [Fe/H] tra -4 e -2}
    \label{fig:Cno_2_4}
\end{figure}


\textcolor{red}{Inizia parte vecchia da eliminare/rivedere}



In figure \ref{fig:onlypopiii_delta} we represent the ISM abundance ratios for some key chemical elements compared to the abundance of iron, $[Fe/H]$, when mini-halos are enriched only by PopIII SNe, using the results of the equations \ref{XsuHiii} and \ref{XsuFeiii}. The plots in the first four columns are for $M_* \in [10; 100] M_{\odot}$ (\emph{normal} SNe range), while the plots in the last column are for $M_* \in [140; 260] M_{\odot}$ (PISN range). Choosing a delta function IMF and dividing the results for different explosion energies, the position of each point in the plots of the figure depends on the initial mass of the stars, represented by the colors (blue for the lighter stars and green for the heavier ones), and the value of $f_*/f_{dil}$. Indeed, if we inspect equations \ref{XsuHiii} and \ref{XsuFeiii} we can see that they depend on $Y_{X}^{PopIII}$, which depends only on the masses of the stars that explode in the mini-halo and their explosion energies, and on $f_*/f_{dil}$, for which we chose ten representative values in the already mentioned range. Different values of $f_*/f_{dil}$ affect $[Fe/H]$, but not $[X/Fe]$. 

We will firstly comment (\textcolor{red}{si dice così?}) on the results we get when $M_* \in [10;100] M_{\odot}$, focusing on the plots in the first four columns on the left. 

The overall trend with increasing explosion energy, increasing from the left to the right columns in figure \ref{fig:onlypopiii_delta}, is an increase in $[Fe/H]$ and a decrease in $[X/Fe]$ for most of the chemical elements. This is due to the fact that low-energy SNe experience a strong fall-back and expel only the most external shells of the star. That's also why $[Fe/H]$ reaches very low values, up to $-8$, only when low-energy SNe explode in the mini-halos. However, the upper limit of $[Fe/H]$ is always $\ge -1$.

Focusing on the lighter elements like C, O and Mg, $[X/Fe] > 3$ can be reached only with the explosions of faint SNe and CC SNe. 



Furthermore, for the same elements, there is a relation between $[X/Fe]$ and the initial mass of the stars which explode in the mini-halo: the more massive is the star, the higher is $[X/Fe]$. This means that, to get a strong enhancement in these elements, only very massive ($M_* > 50 M_{\odot}$) low-energy SNe ($E_{SN} < 2 \times 10^{51} erg$) must explode in the mini-halos. Among the elements we considered, $[Mn/Fe]$ and $[Zn/Fe]$ seem independent on the energy of the SN explosion and the initial mass of the stars, always being between $-1$ and $1$. This may be due to the fact that Mn and Zn are the only chemical elements with production processes similar to the ones of Fe (\textcolor{red}{è vero questo?}).

Let's now inspect the plots in the right column of figure \ref{fig:onlypopiii_delta}, where the initial masses of the stars are between $140 M_{\odot}$ and $260 M_{\odot}$, thus they explode as Pair Instability SN (PISN). In this case the explosion energy is proportional to the initial mass of the stars (from $E_{SN}=10^{52} erg$ for a $140 M_{\odot}$ star to $E_{SN}=10^{53} erg$ for a $260 M_{\odot}$ star). 

For all the chemical elements we considered, a part from Zn, there is a clear relation between $[Fe/H]$, $[X/Fe]$ and the initial mass (or the explosion energy) of the stars: the most massive stars enrich the ISM to higher values of $[Fe/H]$ and to lower values of $[X/Fe]$. This is due to the fact that the amount of Fe synthesized by the stars that explode as PISN is almost proportional to their initial mass, while the amount of the other chemical elements is almost constant for different initial masses (see \citet{Heger2002a} for details). The same relation doesn't hold for $[Zn/Fe]$, which increases for the higher and the lower stellar masses, but decreases for the middle ones, and is always $< -1$. In general PISN produce and expel very little Zn due to the lack of neutron excess.

\subparagraph{The progenitors of CEMP-no stars}

The most Fe-poor and C-enhanced halo stars, with $[Fe/H] < -4$ and $[C/Fe] > 3$, are believed to have just one progenitor, usually a massive ($M_* > 20 M_{\odot}$) primordial faint SNe (see \citet{Iwamoto2005a}, \citet{Keller}). But, if we look at the $[C/Fe]$ diagrams in figure \ref{fig:onlypopiii_delta}, also massive CC SNe or the lightest PISNe can be their progenitors, while HE SNe and hypernovae can be excluded. 

What happens if we consider also the other chemical elements? What we said above holds also for almost all the chemical elements we represented here (a part from Al) for the faint SN and the CC SN cases, but not for the PISN case: with this latter approach we can reproduce the chemical abundances of the most Fe-poor and C-enhanced halo stars just for the elements C, O and Mn. Thus, we can exclude also the lighter PISN as the progenitors of these stars.

However, this kind of parametric study is very simple, indeed we are supposing that just one PopIII star (or more with the same initial mass and explosion energy) forms and explodes in the mini-halos, thus it might also be unrealistic, since various simulations of primordial star formation processes predict that multiple PopIII stars can form.

